Systematic Generalisation through Task Temporal Logic and Deep Reinforcement Learning

This work introduces a neuro-symbolic agent that combines deep reinforcement learning (DRL) with temporal logic (TL) to achieve systematic zero-shot, i.e., never-seen-before, generalisation of formally specified instructions. In particular, we present a neuro-symbolic framework where a symbolic module transforms TL specifications into a form that helps the training of a DRL agent targeting generalisation, while a neural module learns systematically to solve the given tasks. We study the emergence of systematic learning in different settings and find that the architecture of the convolutional layers is key when generalising to new instructions. We also provide evidence that systematic learning can emerge with abstract operators such as negation when learning from a few training examples, which previous research have struggled with.

==> utils/acro_list.tex <==
\begin{acronym}[rPATL] % Give the longest label here so that the list is nicely aligned
\acro{PATL}{Probabilistic Alternating-time Temporal Logic}
\acro{rPATL}{PATL with rewards}
\acro{RL}{reinforcement learning}
\acro{MARL}{Multi-Agent RL}
\acro{IRL}{Inverse RL}
\acro{DRL}{Deep Reinforcement Learning}
\acro{MC}{Model Checking}
\acro{PCTL}{Probabilistic Branching-time Temporal Logic}
\acro{LDL}{Linear Dynamic Logic}
\acro{TL}{Temporal Logic}
\acro{MDP}{Markov Decision Process}
\acro{POMDP}{Partially Observable Markov Decision Process}
\acro{EMDP}{Extended Markov Decision Process}
\acro{pCGS}{probabilistic Concurrent Game Structure}
\acro{MG}{Markov Game}
\acro{EMG}{Extended Markov Game}
\acro{FM}{Formal Methods}
\acro{DL}{Deep Learning}
\acro{$LTL$}{Linear-time Temporal Logic}
\acro{STL}{Signal Temporal Logic}
\acro{DQNs}{Deep Q-Networks}
\acro{HRL}{hierarchical reinforcement learning}
\acro{DFA}{Deterministic Finite Automaton}
\acro{NMRDP}{Non-Markovian Reward Decision Process}
\acro{PONMDP}{Partially Observable Non-Markovian Reward Decision Process}
\acro{MTCLS}{multi-task co-safe LTL specification}
\acro{RM}{Reward Machine}
\acro{NMRG}{Non-Markovian Reward Game}
\acro{SMAC}{StarCraft Multi-Agent Challenge}
\acro{EA}{Evolutionary Algorithm}
\acro{MAS}{Multi-agent System}
\acro{IQL}{Independent Q-Learning}
\acro{AI}{Artificial Intelligence}
\acro{STL}{Signal Temporal Logic}
\acro{I-DQN}{Independent Deep Q-Learning}
\acro{LPOPL}{LTL Progressionfor Off-Policy Learning}
\acro{DL}{Deep Learning}
\acro{ANN}{Artificial Neural Network}
\acro{DNN}{Deep Neural Network}
\acro{CNN}{Convolutional Neural Network}
\acro{ML}{machine learning}
\acrodefplural{NMRDP}[NMRDPs]{Non-Markovian Reward Decision Processes}
\acrodefplural{MG}[MGs]{Markov Games}
\acrodefplural{MDP}[MDPs]{Markov Decision Processes}
\acrodefplural{POMDP}[POMDPs]{Partial Observable Markov Decision Processes}

\end{acronym}

==> utils/table1_copy_.tex <==
\begin{table*}[t]
    \centering
  \mycfs{9}
   \begin{tabular}{lcccccccc}
    \toprule
      & \multicolumn{2}{c}{2L-CNN} &  \multicolumn{2}{c}{ResNet}  & \multicolumn{2}{c}{Env-CNN} 
  & \multicolumn{2}{c}{Env-CNN\textsuperscript{RF}}\\
\cmidrule(r){2-3}
\cmidrule(r){4-5}
\cmidrule(r){6-7}
\cmidrule(r){8-9}
  $|\mathcal{X}_{1}|$ & Train & Test & Train & Test & Train & Test &  Train & Test  \\
% \midrule
  6  & 1.55$(0.14)$ &	1.5$(0.13)$ &	1.91$(0.49)$ & 1.75 $(0.54)$ & \textbf{9.13$(3.46)$} & 2.08$(0.35)$ & 3.59$(2.71)$ & 2.71$(0.58)$\\
  
 10  &2.74$(0.13)$
	& 2.5$(0.13)$ & 2.12$(0.85)$& 1.98$(0.81)$ & 6.91$(2.32)$ &	3.47 $(2.13)$& 
	\textbf{7.87$(1.55)$} & \textbf{3.81$(1.54)$}\\
 20 & 3.39$(0.14)$ & 3.18$(0.15)$	& 2.37$(0.87)$ & 2.32$(0.86)$	& \textbf{9.67$(1.04)$}	& \textbf{8.27$(0.59)$}&	6.65$(1.03)$ & 5.68$(0.64)$ \\
    \bottomrule
  \end{tabular}
   \normalsize
    \caption{Mean and standard deviation from the average rewards obtained from 3 independent runs in a set of 500 maps solving atomic tasks. Values are normalized so that 1.0 is the performance of a random walker.\bg{Vertical, the different CNNs, horizontal Minecraft and Minigrid, with 6 and 20 objects each}} \label{table:tasks}
\end{table*}

==> utils/table2_copy_.tex <==
\begin{table*}[t]

  \centering
    \mycfs{9}
   \begin{tabular}{P{0.6cm}cccccccc}
    \toprule
\textbf{Positive} \\ instructions & \multicolumn{2}{c}{2L-CNN} &  \multicolumn{2}{c}{ResNet}  & \multicolumn{2}{c}{Env-CNN} 
  & \multicolumn{2}{c}{Env-CNN\textsuperscript{RF}}\\
\cmidrule(r){2-3}
\cmidrule(r){4-5}
\cmidrule(r){6-7}
\cmidrule(r){8-9}
  $|\mathcal{X}_{1}|$ & Reliable & Deceptive & Reliable & Deceptive & Reliable & Deceptive &  Reliable & Deceptive  \\
  6  & 2.13 $(0.23)$ & 2.33$(0.57)$
        &	2.72$(0.12)$ & 2.5$(0.69)$ & 4.06$(4.79)$ & 0.35$(0.29)$ & 
        \textbf{12.86}$(9.74)$ &\textbf{0.25$(0.06)$}\\
 10  &4.53$(0.45)$&4.3$(0.49)$&       
        3.25$(1.62)$ 	&        
        3.21$(1.62)$  & \textbf{9.33}$(6.72)$
        & 1.12$(0.95)$& 
        4.44$(5.12)$ &\textbf{0.28$(0.27)$}\\
20 & 7.16$(0.13)$ & 6.93$(0.76)$&     
    3.52$(1.98)$ & 3.52$(1.87)$	& \textbf{18.75}$(2.88)$ &	\textbf{0.11}$(0.03)$  &  
    12.3$(6.21)$ &0.22$(0.1)$\\
    
\midrule    

\textbf{Negative} \\ instructions & \multicolumn{2}{c}{2L-CNN} &  \multicolumn{2}{c}{ResNet}  & \multicolumn{2}{c}{Env-CNN} 
  & \multicolumn{2}{c}{Env-CNN\textsuperscript{RF}}\\
\cmidrule(r){2-3}
\cmidrule(r){4-5}
\cmidrule(r){6-7}
\cmidrule(r){8-9}
  $|\mathcal{X}_{1}|$ & Reliable & Deceptive & Reliable & Deceptive & Reliable & Deceptive &  Reliable & Deceptive  \\
  6  & 2.31$(0.9)$ & 2.36$(0.98)$
        &	2.2$(0.27)$ & 	1.99$(0.31)$ & 1.52$(0.93)$ &0.53$(0.46)$ & 
        \textbf{4.51}$(4.34)$ &\textbf{0.44}$(0.35)$\\
 10  &2.58$(0.18)$&2.94$(0.7)$&       
        2.91$(1.53)$ 	&        
        3.14$(1.7)$  & 3.72$(3.04)$
        & 0.56$(0.27)$& 
        \textbf{5.31}$(4.94)$ &\textbf{0.22}$(0.16)$\\
20 & 5.79$(1.36)$ & 5.91$(1)$&     
    2.38$(1.38)$ & 2.28$(1.72)$	& \textbf{11.26}$(4.69)$ &	\textbf{0.1}$(0.02)$  &  
    4.9$(5.52)$ &0.16$(0.06)$\\
    
 \bottomrule
\end{tabular}
\normalsize
\caption{Results from 500 binary choice maps using zero-shot objects. Agents that are learning systematically should perform well with reliable instructions and poorly with deceptive instructions, i.e., in 'Reliable' higher is better while in 'Deceptive' lower is better. }\label{table:BCMs}
\end{table*}

==> utils/table3.tex <==
\begin{table*}
  \centering
  \small
\begin{tabular}{lcccccccr}
  \toprule
  & \multicolumn{2}{c}{E+MLP} &  \multicolumn{2}{c}{RE+MLP}  & \multicolumn{2}{c}{2-layer CNN} 
  & \multicolumn{2}{c}{ResNet}\\
\cmidrule(r){2-3}
\cmidrule(r){4-5}
\cmidrule(r){6-7}
\cmidrule(r){8-9}
  $|\mathcal{X}_{1}|$ & Positive & Negative & Positive & Negative & Positive & Negative &  Positive & Negative  \\
  6  & -15.09\scriptsize$\pm2.87$ &	-4.13\scriptsize$\pm1.38$ &	-22.04\scriptsize$\pm1.1$& -0.01\scriptsize$\pm0.15$  &   
        -0.48\scriptsize$\pm0.29$  &	0.20\scriptsize$\pm0.42$  & 0.58\scriptsize$\pm0.39$  &	0.68\scriptsize$\pm0.51$\\
 10  &-14.39\scriptsize$\pm3.08$ & -3.72\scriptsize$\pm0.81$ & -23.29\scriptsize$\pm1.78$ & -1.69\scriptsize$\pm0.97$  & 0.9\scriptsize$\pm0.41$ 
        & 0.89\scriptsize$\pm0.24$  & 0.22\scriptsize$\pm0.61$  &	0.66\scriptsize$\pm0.51$\\
 20 & -14.41\scriptsize$\pm2.37$ & -3.26\scriptsize$\pm0.54$ & -17.84\scriptsize$\pm6.25$
    & -0.71\scriptsize$\pm0.41$ & -0.32\scriptsize$\pm0.60$ & 1.29\scriptsize$\pm0.67$   & 0.88\scriptsize$\pm0.44$  &	1.76\scriptsize$\pm0.49$\\
\bottomrule
\end{tabular}
\caption{Rewards obtained in the 500 binary choice maps with deceptive instructions. Here lower is better.}
\label{table:BCFake}
\end{table*}

==> utils/table4.tex <==
\begin{table}
  \centering
  \small
\begin{tabular}{M{0.7cm}M{1.3cm}M{1.3cm}M{1.3cm}M{1.1cm}} 
\toprule
  & 1-layer CNN &  LSTM  & 2-layer CNN & Random walker\\
\midrule
Train & 7.42\tiny$\pm0.05$ &7.49\tiny$\pm0.18$ & 7.42\tiny$\pm0.0$ & 3.98\tiny$\pm0.1$\\
Test  & 6.25\tiny$\pm0.49$ & 6.94\tiny$\pm0.17$ & 3.84\tiny$\pm0.34$ & 3.98\tiny$\pm0.1$ \\
\bottomrule
\end{tabular}
\caption{Rewards obtained in 2k maps with subtasks using positive, negative and non-deterministic choice operators.}
\label{table:FullVocabA}
\end{table}

